PILArNet: Public Dataset for Particle Imaging Liquid Argon Detectors in High Energy Physics

Rapid advancement of machine learning solutions has often coincided with the production of a test public data set. Such datasets reduce the largest barrier to entry for tackling a problem -- procuring data -- while also providing a benchmark to compare different solutions. Furthermore, large datasets have been used to train high-performing feature finders which are then used in new approaches to problems beyond that initially defined. In order to encourage the rapid development in the analysis of data collected using liquid argon time projection chambers, a class of particle detectors used in high energy physics experiments, we have produced the PILArNet, first 2D and 3D open dataset to be used for a couple of key analysis tasks. The initial dataset presented in this paper contains 300,000 samples simulated and recorded in three different volume sizes. The dataset is stored efficiently in sparse 2D and 3D matrix format with auxiliary information about simulated particles in the volume, and is made available for public research use. In this paper we describe the dataset, tasks, and the method used to procure the sample.

==> old.tex <==
\bibitem{AlexNet}
A. Krizhevsky, I. Sutskever, G. Hinton, ``ImageNet Classification with Deep Convolutional Neural Networks,'' \emph{proceedings of the NIPS}, {\bf{1}}, 1097-1105 (2012).

\bibitem{NatureDeepLearning}
Y. LeCun, Y. Bengio, G. Hinton, ``Deep learning,'' Nature {\bf 521} p.436-444 (2015).

\bibitem{MNIST}
LeCun, Y., Bottou, L., Bengio, Y., and Haffner, P., ``Gradient-based learning applied to document recognition,'' \emph{proceedings of the IEEE}, {\bf{86}}, 2278–2324 (1998).

\bibitem{CIFAR}
Alex Krizhevsky, Vinod Nair and Geoffrey Hinton, ``CIFAR-10 (Canadian Institute for Advanced Research),'' \protect\url{http://www.cs.toronto.edu/~kriz/cifar.html}

\bibitem{ImageNet}
O. Russakovsky, J. Deng, H. Su, J. Krause, S. Satheesh, S. Ma, Z. Huang, A. Karpathy, A. Khosla, M. Bernstein, A.  Berg, and L. Fei-Fei, ``ImageNet Large Scale Visual Recognition Challenge,'' \emph{International Journal of Computer Vision (IJCV)}, {\bf{115}}, 3, 211-252 (2015).

\bibitem{COCO}
T.-Y. Lin, M. Marie, S. Belongie, L. Bourdev, R. Girshick, J. Hays, P. Perona, D. Ramanan, C. L. Zitnick, P. Dollár, ``Microsoft COCO: Common Objects in Context,'' \emph{arXiv:1405.0312} [cs.CV] (2014).

\bibitem{PASCAL}
M. Everingham, L. Van Gool, C. K. I. Williams, J. Winn, and A. Zisserman, ``The PASCAL Visual Object Classes (VOC) Challenge,'' \emph{International Journal of Computer Vision}, {\bf{88}}(2), 303-338 (2010).


\bibitem{ShapeNet}
A. X. Chang, T. Funkhouser, L. Guibas, P. Hanrahan, Q. Huang, Z. Li, S. Savarese, M. Savva, S. Song, H. Su, J. Xiao, L. Yi, and F. Yu, ``ShapeNet: An Information-Rich 3D Model Repository,'' \emph{arXiv:1512.03012} [cs.GR] (2015).

\bibitem{UBPaper1}
R. Acciarri et al. (MicroBooNE Collaboration), ``Convolutional neural networks applied to neutrino events in a liquid argon time projection chamber,'' \emph{Journal of Instrumentation} \textbf{12}, no.03, P03011 (2017).

\bibitem{UBPaper2}
C. Adams et al. (MicroBooNE Collaboration), ``
A Deep Neural Network for Pixel-Level Electromagnetic Particle Identification in the MicroBooNE Liquid Argon Time Projection Chamber,'' \emph{arXiv:1808.07269} [phys.Ins-det] (2018).

\bibitem{UBNature}
A. Radovic, M. Williams, D. Rousseau, M. Kagan, D. Bonacorsi, A. Himmel, A. Aurisano, K. Terao, T. Wongjirad, ``Machine learning at the energy and intensity frontiers of particle physics,'' \emph{Nature} \textbf{volume 560}, pages 41--48 (2018).

\bibitem{UBDetector}
R. Acciarri et al. (MicroBooNE Collaboration), ``Design and construction of the MicroBooNE detector,'' \emph{Journal of Instrumentation} \textbf{12}, 02017 (2017).

\bibitem{SBN}
M. Antonello et al. (MicroBooNE, LAr1-ND, and ICARUS-WA104 Collaboration),
``A Proposal for a Three Detector Short-Baseline Neutrino Program in the Fermilab Booster Neutrino Beam,''
\emph{arXiv:1503.01520} [physics.ins-det].

\bibitem{DUNE}
R. Acciarri et al. (DUNE Collaboration),
  ``Long-Baseline Neutrino Facility (LBNF) and Deep Underground Neutrino Experiment (DUNE) : Volume 1: The LBNF and DUNE Projects,'' \emph{arXiv:1601.05471} [physics.ins-det].
  
\bibitem{ArgonCube}
A. Ereditato et al. (ArgonCube Collaboration), ``ArgonCube: a Modular Approach for Liquid Argon TPC Neutrino Detectors for Near Detector Environments,'' SPSC-I-246 (2017) \protect\url{https://cds.cern.ch/
record/2268439/files/SPSC-I-246.pdf}.

\bibitem{LArPix}
D. A. Dwayer, M. Garcia-Sciveres, D. Gnani, C. Grace, S. Kohn, M. Kramer, A. Krieger, C. J. Lin, K. B. Luk, ``LArPix: demonstration of low-power 3D pixelated charge readout for liquid argon time projection chambers,'' \emph{Journal of Instrumentation} \textbf{13}, no.13, P10007 (2018)

\bibitem{Geant4}
S. Agostinelli et al., ``GEANT4: A Simulation toolkit,''
{\it NIM} {\bf A506} 250-303, 2003.

\bibitem{LArSoft}
E. L. Snider et al., ``LArSoft: Toolkit for Simulation, Reconstruction and Analysis of Liquid Argon TPC Neutrino Detectors,'' \emph{J.Phys.Conf.Ser.} \textbf{898} no.4 (2017).

\bibitem{Generator}
LArTPC Custom Event Generator (DeepLearnPhysics) \protect{\url{https://github.com/DeepLearnPhysics/LArTPCEventGenerator}}

\bibitem{PubPAID}
DeepLearnPhysics organization, ``Public PArticle Imaging Dataset (PubPAID) by DeepLearnPhysics,'' \protect{\url{https://osf.io/tswnx/}}.

\bibitem{PubLAr}
DeepLearnPhysics organization, ``LArTPC 2D/3D - Simulation - Particle Segmentation \& Clustering,'' \protect{\url{https://osf.io/vruzp/}}.

\bibitem{LArCV}
LArCV: Liquid Argon and Computer Vision Software (DeepLearnPhysics) \protect{\url{https://github.com/DeepLearnPhysics/larcv2}}.

\bibitem{Docker}
D. Merkel, ``Docker: Lightweight Linux Containers for Consistent Development and Deployment,'' \emph{Linux J.} \textbf{2}, 239 (2014).

\bibitem{Singularity}
G. M. Kurtzer, V. Sochat, M. W. Bauer, ``Singularity: Scientific containers for mobility of compute,'' \emph{PLoS ONE} \textbf{12(5)}, e0177459 (2017). \protect{\url{https://doi.org/10.1371/journal.pone.0177459}}

\bibitem{SingularityHub}
G. M. Kurtzer, C. J. Prybol, G. M. Kurtzer, ``Enhancing reproducibility in scientific computing: Metrics and registry for Singularity containers,'' \emph{PLoS ONE} \textbf{12(11)}, e0188511 (2017). \protect{\url{https://doi.org/10.1371/journal.pone.0188511}}

\bibitem{DLPDocker}
DeepLearnPhysics Docker-Hub Repository \protect{\url{https://cloud.docker.com/u/deeplearnphysics/repository/docker/deeplearnphysics/larcv2}}

\bibitem{DLPSingularity}
DeepLearnPhysics Singularity-Hub Repository \protect{\url{https://www.singularity-hub.org/collections/459}}

\bibitem{DockerRecipe}
DeepLearnPhysics Docker Recipes Repository \protect{\url{https://github.com/DeepLearnPhysics/larcv2-docker}}

\bibitem{SingularityRecipe}
DeepLearnPhysics Docker Recipes Repository \protect{\url{https://github.com/DeepLearnPhysics/larcv2-singularity}}

\bibitem{APIs}
DeepLearnPhysics Open Data APIs \protect{\url{https://github.com/DeepLearnPhysics/dlp_opendata_api}}

\bibitem{LArCVTutorial}
DeepLearnPhysics LArCV Tutorial  \protect{\url{http://deeplearnphysics.org/Blog/tutorial_summary.html#tutorial_summary}}


